Immersions of $C_2$-projective spaces via $K\mathbb{R}$-theory

We compute the Atiyah Real $K$-theory of $C_2$-equivariant projective spaces and construct immersions of such spaces into multiples of the regular representation. These computations are made tractable by the recent geometric filtration of equivariant projective spaces due to Bhattacharya-Waugh-Zeng-Zou, together with a variant of the localized slice spectral sequence introduced by Meier-Shi-Zeng. As an immediate corollary of these computations, we obtain an equivariant analogue of James periodicity.

==> not_used.tex <==
The goal of this section is to compute the homotopy groups of $k_\r \wedge B_{C_2} \Sigma_2$. The strategy is same as in the $H \underline{\z}$-case: we need the Thom isomorphism to reduce the $k_\r$-homology of the Thom space to something more tractable, and then apply the Atiyah-Hirzebruch spectral sequence to obtain the final answer. The first step is to check the orientability of the tautological bundle in the spectrum $K_\r$. The case of $k_\r$ then follows immediately.

\begin{proposition}
    $n \widetilde{\gamma_{\rho}^{(k)}}$ is $K_\r$-orientable.
\end{proposition}
\begin{proof}
    
\end{proof}

\begin{corollary}[Thom isomorphism] \label{K_R Thom iso}
    
\end{corollary}

\todo[inline]{Albert: To modify below.}

For any $V \in RO(C_2)$, \cref{filtration of BC_2 C_2} now gives rise to a spectral sequence after wedging $k_{\r}$ to the whole filtration, whose $E^1$-page is $$E_{n, V}^1 = {(k_{\r})}_V \left ( \Th(n \widetilde{\gamma_{\rho}^{(1)}}) \right ) \Rightarrow (k_\r)_V (B_{C_2} \Sigma_2).$$ The $d_1$-differentials is given by $d_1: E_{n, V}^1 \to E_{n-1, V}^1$. By \cref{K_R Thom iso}, $$E_{n, V}^1 \cong (k_{\r})_{V - n\rho} (S^\sigma \vee S^0) = (k_{\r})_{V - n\rho - \sigma} \{ e_{\sigma}^{(n)} \} \oplus (k_{\r})_{V - n\rho} \{ e_{0}^{(n)} \},$$ where $e_{\sigma}^{(n)}$ and $e_{0}^{(n)}$ are the generators of $S^{\sigma}$ and $S^0$ in filtration $n$, respectively. By Bott periodicity, the $RO(C_2)$-grading for $k_{\r}$ descents to the usual $\n$-grading, so it is safe to set $V = a+ b\sigma$ for $a, b \in \n$, and note that $(k_\r)_V \cong (k_\r)_{a-b}$. To determine the $d_1$-differential, we take the restrictions maps to both ends
\[
    \begin{tikzcd}
        (k_{\r})_{V - n\rho - \sigma} \{ e_{\sigma}^{(n)} \} \oplus (k_{\r})_{V - n\rho} \{ e_{0}^{(n)} \} \arrow[r, "d_1"] \arrow[d, "\text{res}_{e}^{C_2}"'] & (k_{\r})_{V - (n-1)\rho - \sigma} \{ e_{\sigma}^{(n-1)} \} \oplus (k_{\r})_{V - (n-1)\rho} \{ e_{0}^{(n-1)} \} \arrow[d, "\text{res}_{e}^{C_2}"] \\
        (ku)_{a+b - (2n + 1)} \{ e_{\sigma}^{(n)} \} \oplus (ku)_{a+b - 2n} \{ e_{0}^{(n)} \} \arrow[r, "d_1"] \arrow[d] & (ku)_{a+b - (2n - 1)} \{ e_{\sigma}^{(n)} \} \oplus (ku)_{a+b - (2n-2)} \{ e_{0}^{(n)} \} \arrow[d] \\
        (H\z)_{a+b - (2n + 1)} \{ e_{\sigma}^{(n)} \} \oplus (H\z)_{a+b - 2n} \{ e_{0}^{(n)} \} \arrow[r, "d_1"] & (H\z)_{a+b - (2n - 1)} \{ e_{\sigma}^{(n)} \} \oplus (H\z)_{a+b - (2n-2)} \{ e_{0}^{(n)} \} 
    \end{tikzcd}
\]

Taking the slices of both sides of $d_1$ (depicted in the bottom row of the commutative diagram), we can take a close observation of how $d_1$ acts on the generators. Recall that $\p((n \rho)$ is obtained from $\p((n-1) \rho)$ by attaching a total disk bundle $D(n \widetilde{\gamma_{\rho}^{(1)}})$ via the projection $\text{proj}_n: S(n \widetilde{\gamma_{\rho}^{(1)}})) \to \p((n-1) \rho)$. Fiberwise, the attaching map $\text{proj}_n$ is 2-fold covering map. Explicitly, two cells $e_{\sigma}^{(n)}$ and $e_{0}^{(n)}$ of $\p(n \rho)$ are attached to $e_{\sigma}^{(n-1)}$ and $e_{0}^{(n-1)}$ of $\p((n-1) \rho)$, and the $e_{0}^{(n)}$ is attached to $e_{\sigma}^{(n-1)}$ via a degree 2 map. Thus, 
\begin{equation} \label{eq: d_1 differential k_R}
    d_1(e_{0}^{(n)}) = e_{\sigma}^{(n-1)}, \quad d_1(e_{\sigma}^{(n)}) = 0.
\end{equation}    
By the commutativity of the diagram, the same $d_1$-action on the generators also obey the same rule in $ku_*$-homology and hence in ${(k_\r)}_V$-homology. Therefore, we completely determine the $E^1$-page of the spectral sequence. 

\begin{figure}[H]
\includegraphics[scale=.9]{pictures pdf/fil n.pdf}
\includegraphics[scale=.9]{pictures pdf/fil n-1.pdf}
\caption{The diagram illustrates the $n$-th (upper) and $(n-1)$-st (lower) filtrations of the spectral sequence. The solid squares represent the $(k_\r)_*$-classes in the current ($n$-th) filtration, while the hollow squares represent $(k_\r)_*$-classes in the adjacent (lower) filtration. For example, in the $n$-th (upper) filtration, the solid squares correspond to elements in \( E_{n,V}^1 \), whereas the hollow squares indicate elements in \( E_{n-1,V}^1 \), which do not appear in \( E_{n,V}^1 \) itself. We retain the hollow squares solely to visualize the $d_1$-differentials between the two filtrations.}\label{fig:fil n and n-1}. 
\end{figure}

Note that since $k_\r$ is connective, there is nothing strictly below the line $a+b = 2n$ in filtration $n$, as shown in \cref{fig:fil n and n-1}. These lines are called the \textbf{vanishing lines}. Hence, we can restrict our attention to the part above such vanishing lines in each filtration. To examine the spectral sequence in detail, we observe that each element on the $E^1$-page appears in pairs, as illustrated by the solid and hollow squares in \cref{fig:fil n and n-1}. In each pair, the upper square represents the contribution from $S^0$, while the lower square represents the contribution from $S^{\sigma}$. By \cref{eq: d_1 differential k_R}, we see that the $d_1$-differentials map the lower squares in filtration $n$ to the upper squares in filtration $n-1$ via a degree $2$ map. That is, $d_1$ should go from the upper diagram in \cref{fig:fil n and n-1} to the lower diagram. 

Since $a$ and $b$ vary in $\z$, each point strictly above the vanishing line can arise either from $S^0$ or from $S^{\sigma}$. To simplify the discussion, we adopt the notation $\blacktriangledown$ to denote the pair $(k_{\r})_{V - n\rho - \sigma} \{ e_{\sigma}^{(n)} \} \oplus (k_{\r})_{V - n\rho} \{ e_{0}^{(n)} \}$, and place it at the position corresponding to the contribution from $S^0$. Namely,
\[
    \scalebox{3}{$\blacktriangledown$}_{= (k_{\r})_{V - n\rho - \sigma} \{ e_{\sigma}^{(n)} \}}^{= (k_{\r})_{V - n\rho - \sigma} \{ e_{0}^{(n)} \}}
\]
By doing this, we obtain the nice pictures of $E_{n, V}^1$ and $E_{n-1, V}^1$, as shown in \cref{fig:improved fil n and n-1}, with each grid point having at most one signature.

\begin{figure}[H]
\includegraphics[scale=.9]{pictures pdf/improved fil n.pdf}
\includegraphics[scale=.9]{pictures pdf/improved fil n-1.pdf}
\caption{The diagram illustrates the $n$-th (upper) and $(n-1)$-st (lower) filtrations of the spectral sequence using the adapted notion $\blacktriangledown$. The hollow squares $\square$ indicate “half” of a $\blacktriangledown$; that is, only the part corresponding to the contribution from $S^0$ is present.}\label{fig:improved fil n and n-1}. 
\end{figure}

From the previous discussion, we see that the $d_1$-differentials go from the $n$-th filtration (the upper diagram in \cref{fig:improved fil n and n-1}) to the $(n-1)$-th filtration (the lower diagram in \cref{fig:improved fil n and n-1}), moving one unit to the left and one unit down. On the vanishing lines, we observe that the contributions from $S^{\sigma}$ cannot survive due to connectivity. Therefore, only half of the information remains, and all surviving classes are targets of the $d_1$-differentials.


% We adapt the following notions for the relevant $C_2$-equivariant Mackey functor:
% \[
%     \renewcommand{\arraystretch}{1.5}
%     \begin{array}{*{3}{>{\centering\arraybackslash}m{3cm}}}
%         \bullet & \square & \blacksquare \\
%         \tikz[baseline=(Z2.base)]{
%             \node (Z2) at (0,1.0) {$\z/2$};
%             \node (zero) at (0,0) {$0$};
%             \draw[->, bend left=30] (Z2) to (zero);
%             \draw[->, bend left=30] (zero) to (Z2);
%                 }
%         &
%         \tikz[baseline=(Z2.base)]{
%             \node (Z2) at (0,1.0) {$0$};
%             \node (zero) at (0,0) {$\z_-$};
%             \draw[->, bend left=30] (Z2) to (zero);
%             \draw[->, bend left=30] (zero) to (Z2);
%                 } 
%         &
%         \tikz[baseline=(Z2.base)]{
%             \node (Z2) at (0,1.0) {$\z$};
%             \node (zero) at (0,0) {$\z$};
%             \draw[->, bend left=30] (Z2) to node[right]{\scriptsize $1$} (zero);
%             \draw[->, bend left=30] (zero) to node[left]{\scriptsize $2$} (Z2);
%                 }
%     \end{array}
% \]

% The notation $\mathbb{Z}_-$ denotes a $\mathbb{Z}[C_2]$-module, where the $C_2$-action on the basis elements $\mathbb{Z}\{x^i\}$, for the generator $x$, is given by multiplication by $(-1)^i$; in particular, the action is by $-1$ when $i$ is odd. 


Following Beaudry's note \cite{Beaudry_note}, we present the result for $(K_\r)_*$ in Dugger's thesis \cite{Dugger} in the following picture for completeness. The result for the connective cover $k_{\r}$ is simply forgetting the negative cone. 

\begin{figure}[H]
\includegraphics[scale=.75]{pictures pdf/complete K_R.pdf}
\caption{The $E_3$-page of the slice spectral sequence computing $K_\r$. The green arrows are $d_3$-differentials and the dashed purple line is the exotic transfer, guaranteed by Bott periodicity. Each square (hollow/solid) represents $\z$ and each dot (hollow/solid) represents $\z/2$.}\label{fig:k_R}. 
\end{figure}

Note that in the spectral sequence, $u_{2 \sigma}$ supports a $d_3$-differential $$d_3(u_{2 \sigma}) = \overline{v_1} a_{\sigma}^3, $$ which is linear with respect to $\overline{v_1}$, where the latter one is a permanent cycle. The classes $\overline{v_1}, u_{2 \sigma}$ are furthermore units in $K_{\r}$, so $$d_3 \left (\frac{u_{2 \sigma}}{\overline{v_1}} \right ) = a_{\sigma}^3.$$ Write $$\alpha = \overline{v_1}^2 u_{2\sigma}, \quad \beta = \overline{v_1} a_{\sigma}.$$ For every $j, k \geq 1$, we write $$g_k = \frac{2}{\overline{v_1}^{2k} u_{2\sigma}^k}, \quad \tau_{k, j} = \frac{\theta}{\overline{v_1}^{2k+1} u_{2\sigma}^{k-1} \cdot \overline{v_1}^j a_{\sigma}^j}.$$ In the negative cone, one directly read from \cref{fig:k_R} that only $\tau_{k,0}$, $\tau_{k,1}$ and $\tau_{k,2}$ survive the $d_3$-differentials for all $k \geq 1$. The usual multiplication structure gives 
\[
    \overline{v_1} a_{\sigma} \cdot \tau_{k,j+1} = \tau_{k,j}.
\]
Note that the hidden extension forces the resulting groups in stem $t-s = -8k$ to be $\z$. Take $G_k$ to be the generator of this $\z$ at stem $t-s=-8k$. We deduce that
\[
    2G_k = g_{2k}.
\]
It follows that
\begin{align} \label{result for K_R} 
    (K_\r)_\star &= (\text{positive cone}) + (\text{negative cone}) \\
        & = \frac{\z[ \alpha, \beta]}{(\beta^3, \alpha \beta, 2\beta)} \oplus \frac{\z \left \{ g_{k}, \tau_{k,j}, G_k \right \}_{k \geq 1, 0 \leq j \leq 2}}{(2G_k - g_{2k}, 2 \tau_{k,j}, \overline{v_1} a_{\sigma} \cdot \tau_{k,j+1} - \tau_{k,j})}, 
\end{align}
where $|a_{\sigma}| = (-\sigma , 1)$, $|\overline{v_1}| = (1+\sigma, 0)$, $|u_{2\sigma}| = (2 - 2\sigma, 0)$, and $|\theta| = (-3+3\sigma, 0)$. Denote $C_{KR} = \coker((K_\r)_{\star} \xrightarrow{2} (K_\r)_\star)$ and $K_{KR} = \ker((K_\r)_\star \xrightarrow{2} (K_\r)_\star)$. In \cref{result for K_R}, it is clear that $\\beta$ and $\tau_{k,j}$ are 2-torsions, so
\[
    K_{KR} \cong \f_2\{ \beta, \beta^2 \} \oplus \frac{\f_2 \{ \tau_{k,j} \}_{k \geq 1, 0 \leq j \leq 2}}{(\overline{v_1} a_{\sigma} \cdot \tau_{k,j+1} - \tau_{k,j})}.
\]
On the other hand, $C_{KR} = (K_\r)_\star \otimes_{\z} \f_2$. It follows that
\[
    C_{KR} \cong \frac{\f_2[ \alpha, \beta]}{(\beta^3, \alpha \beta)} \oplus \frac{\f_2 \left \{ g_{2k-1}, \tau_{k,j}, G_k \right \}_{k \geq 1, 0 \leq j \leq 2}}{(\overline{v_1} a_{\sigma} \cdot \tau_{k,j+1} - \tau_{k,j})}.
\]

Assembling the results together yields
\begin{align} \label{eq: C_KR and K_KR}
    & C_{KR} \cong \frac{\f_2[ \alpha, \beta]}{(\beta^3, \alpha \beta)} \oplus \frac{\f_2 \left \{ g_{2k-1}, \tau_{k,j}, G_k \right \}_{k \geq 1, 0 \leq j \leq 2}}{( \overline{v_1} a_{\sigma} \cdot \tau_{k,j+1} - \tau_{k,j})}, \\
    & K_{KR} \cong \f_2\{ \beta, \beta^2 \} \oplus \frac{\f_2 \{ \tau_{k,j} \}_{k \geq 1, 0 \leq j \leq 2}}{(\overline{v_1} a_{\sigma} \cdot \tau_{k,j+1} - \tau_{k,j})}.
\end{align} 

% Now each $d_1$-differential $d_1: \blacktriangledown \to \blacktriangledown$ in \cref{fig:improved fil n and n-1} is a degree-2 map of Mackey functors in \cref{fig:k_R}. On the level of each components, one has the following:
% \begin{enumerate}
%     \item In the case of $\bullet$,
%         \[
%             \begin{tikzcd}
%                 \z/2 \arrow[d, bend left = 30] \arrow[r, "0"] & \z/2 \arrow[d, bend left = 30] \arrow[r] & \z/2 \arrow[d, bend left = 30] \\ 
%                 0 \arrow[u, bend left = 30] \arrow[r] & 0 \arrow[u, bend left = 30] \arrow[r] & 0 \arrow[u, bend left = 30]
%             \end{tikzcd}
%         \]
%         So the cokernel is $\bullet$ itself.
%     \item In the case of $\square$,
%         \[
%             \begin{tikzcd}
%                 0 \arrow[d, bend left = 30] \arrow[r] & 0 \arrow[d, bend left = 30] \arrow[r] & 0 \arrow[d, bend left = 30] \\ 
%                 \z_- \arrow[u, bend left = 30] \arrow[r, "2"] & \z_- \arrow[u, bend left = 30] \arrow[r] & \z_-/2 \z_- \arrow[u, bend left = 30]
%             \end{tikzcd}
%         \]
%         Since the $C_2$-action on each quotient class $[g] \in \z_-/2 \z_-$ is given by
%         \[
%             a \cdot [g] = [a \cdot g] = [\pm g] = [g] \mod 2
%         \]
%         for each $a \in C_2$, the $C_2$-action is free. The cokernel is 
%             $\tikz[baseline=(Z2.base)]{
%             \node (Z2) at (0,1.0) {$0$};
%             \node (zero) at (0,0) {$\z/2$};
%             \draw[->, bend left=30] (Z2) to (zero);
%             \draw[->, bend left=30] (zero) to (Z2);
%                 } $. We denote it by $\circ$.
                
%     \item In the case of $\blacksquare$,
%         \[
%             \begin{tikzcd}
%                 \z \arrow[d, bend left = 30, "1"] \arrow[r, "2"] & \z \arrow[d, bend left = 30, "1"] \arrow[r] & \z/2 \arrow[d, bend left = 30, "1"] \\ 
%                 \z \arrow[u, bend left = 30, "2"] \arrow[r, "2"] & \z \arrow[u, bend left = 30, "2"] \arrow[r] & \z/2 \arrow[u, bend left = 30, "0"]
%             \end{tikzcd}
%         \]
%         The resulting cokernel is then $\tikz[baseline=(Z2.base)]{
%             \node (Z2) at (0,1.0) {$\z/2$};
%             \node (zero) at (0,0) {$\z/2$};
%             \draw[->, bend left=30] (Z2) to node[right]{\scriptsize $1$} (zero);
%             \draw[->, bend left=30] (zero) to node[left]{\scriptsize $0$} (Z2);
%                 } $. We denote it by $\diamond$.
% \end{enumerate}

% Hence the cokernel of the $d_1$-differential is given by the following diagram.

% \begin{figure}[H]
% \includegraphics[scale=.9]{pictures pdf/cokernal of d1.pdf}
% \caption{The slice spectral sequence computing the cokernel of $d_1$. The dashed line is an exotic transfer.}\label{fig:cokernal of d1}. 
% \end{figure}

We denote $\triangledown \coloneqq \coker d_1$. The resulting $E^2$-page of the spectral sequence in filtration $(n-1)$ is depicted in \cref{fig:E^2-page}. Explicitly,
\[
    E_{n, \star}^2(K_{\r}) = ({K_\r})_{\star} \{ e_0^{(0)} \} \oplus C_{KR} \{ e_{n \rho + \sigma}^{(n)} \} \oplus K_{KR} \{ e_{n \rho}^{(n)} \}.
\]

\begin{figure}[H]
\includegraphics[scale=.9]{pictures pdf/E^2-page.pdf}
\caption{The diagram illustrates the $(n-1)$-st filtrations of the spectral sequence using the adapted notion $\blacktriangledown$ and $\triangledown$.}\label{fig:E^2-page}. 
\end{figure}

% \begin{proposition}
%     All higher differentials $d_r$ vanishes for $r \geq 2$. Thus, the spectral sequence collapses at $E^2$-page.
% \end{proposition}
% \begin{proof}
%     Similar to \cref{prop: dr die in HZ}, we have a map of spectral sequences $F'_{n, \star}: E_{n, \star}^2(K_\r) \to E_{n, \star}^2(H \underline{\z})$ induced by the augmentation $K_\r \to H \underline{\z}$. Suppose there are nontrivial $d_r$-differentials in $E_{n, \star}^r(K_\r)$. These differentials will descend to ones in $E_{n, \star}^r(H \underline{\z})$, which are trivial by \cref{prop: dr die in HZ}.
% \end{proof}
